UniTRec: A Unified Text-to-Text Transformer and Joint Contrastive Learning Framework for Text-based Recommendation

Prior study has shown that pretrained language models (PLM) can boost the performance of text-based recommendation. In contrast to previous works that either use PLM to encode user history as a whole input text, or impose an additional aggregation network to fuse multi-turn history representations, we propose a unified local- and global-attention Transformer encoder to better model two-level contexts of user history. Moreover, conditioned on user history encoded by Transformer encoders, our framework leverages Transformer decoders to estimate the language perplexity of candidate text items, which can serve as a straightforward yet significant contrastive signal for user-item text matching. Based on this, our framework, UniTRec, unifies the contrastive objectives of discriminative matching scores and candidate text perplexity to jointly enhance text-based recommendation. Extensive evaluation shows that UniTRec delivers SOTA performance on three text-based recommendation tasks. Code is available at https://github.com/Veason-silverbullet/UniTRec.

==> algorithms/rank_algo1.tex <==
\begin{algorithm}[h]
\caption{Ordinal Average Ranking}
\label{alg:rank1}
\begin{algorithmic}[1]
\algsetup{linenosize=\small}
\small
\REQUIRE discriminative scores $S^d=\{S^d_1,S^d_2,...,S^d_M\}$, \\
         \quad\ perplexity-based scores $S^p=\{S^p_1,S^p_2,...,S^p_M\}$.
\ENSURE final averaged ranking $\bar{R}$.

\STATE Sort $S^d$ in ascending order to derive the corresponding ordinal ranking: $R^d\gets\mathrm{Rank_{asc}}(S^d)$.

\STATE Sort $S^p$ in ascending order to derive the corresponding ordinal ranking: $R^p\gets\mathrm{Rank_{asc}}(S^p)$.

\STATE Regard $R^d$ and $R^p$ as scores of rank~(lower for better), average the two ordinal rankings as $\bar{S}\gets(R^d + R^p) / 2$.

\STATE Sort the averaged rankings $\bar{S}$ by descending order to derive the final ranking: $\bar{R}\gets\mathrm{Rank_{des}}(\bar{S})$

\RETURN $\bar{R}$

\end{algorithmic}
\end{algorithm}
